Assessing the Viability of Wave Field Synthesis in VR-Based Cognitive Research

This paper investigates the viability of Wave Field Synthesis (WFS) for enhancing auditory immersion in VR-based cognitive research. While Virtual Reality (VR) offers significant advantages for studying human perception and behavior, auditory cues are often underutilized. WFS, an advanced audio rendering technique, can create highly realistic and spatially accurate soundscapes, potentially increasing ecological validity. This study evaluates WFS by implementing a sample experiment where participants localize static and moving sound sources in both a WFS-rendered environment and a conventional stereo headphone setup. The research explores the impact of virtual environments, sound types, and durations on localization accuracy and search behavior. Findings indicate that while stereo setups can achieve higher accuracy, WFS provides a more natural and intuitive auditory experience, particularly for directional cues. The study also highlights limitations of current WFS systems, such as the lack of height localization, occlusion simulation, and user-dependent optimization, which affect performance, especially for centrally located sound sources. Despite these challenges, WFS shows promise for specialized auditory perception research, particularly for complex soundscapes where directional information is paramount.

==> header_biblatex.tex <==
\usepackage[defernumbers=true,backend=biber,sorting=none,isbn=false,url=false,maxbibnames=999,maxcitenames=2,doi=false,giveninits=true,sortcites=true,citestyle=numeric-comp,eprint=false,hyperref=true]{biblatex}

% reduce size
\AtBeginBibliography{\footnotesize}
\setlength\bibitemsep{0.0\itemsep}

% hide unnecessary fields
\AtEveryBibitem{%
  \clearfield{note}%
}
\AtEveryBibitem{\clearfield{month}}
\AtEveryBibitem{\clearfield{day}}

% display all names when using fullcite
\preto\fullcite{\AtNextCite{\defcounter{maxnames}{99}}}

% allow for bold names
\makeatletter
\def\nhblx@bibfile@name{\jobname -nhblx.bib}
\newwrite\nhblx@bibfile
\immediate\openout\nhblx@bibfile=\nhblx@bibfile@name

\immediate\write\nhblx@bibfile{%
  @comment{Auto-generated file}\blx@nl}

\newcounter{nhblx@name}
\setcounter{nhblx@name}{0}

\newcommand*{\nhblx@writenametobib}[1]{%
  \stepcounter{nhblx@name}%
  \edef\nhblx@tmp@nocite{%
    \noexpand\AfterPreamble{%
      \noexpand\setbox0\noexpand\vbox{%
        \noexpand\nhblx@getmethehash{nhblx@name@\the\value{nhblx@name}}}}%
  }%
  \nhblx@tmp@nocite
  \immediate\write\nhblx@bibfile{%
    @misc{nhblx@name@\the\value{nhblx@name}, author = {\unexpanded{#1}}, %
          options = {dataonly=true},}%
  }%
}

\AtEndDocument{%
  \closeout\nhblx@bibfile}

\addbibresource{\nhblx@bibfile@name}

\newcommand*{\nhblx@boldhashes}{}
\DeclareNameFormat{nhblx@hashextract}{%
  \xifinlist{\thefield{hash}}{\nhblx@boldhashes}
    {}
    {\listxadd{\nhblx@boldhashes}{\thefield{hash}}}}

\DeclareCiteCommand{\nhblx@getmethehash}
  {}
  {\printnames[nhblx@hashextract][1-999]{author}}
  {}
  {}

\newcommand*{\addboldbibnames}{\forcsvlist\nhblx@writenametobib}
\newcommand*{\resetboldbibnames}{\def\nhblx@boldhashes{}}

\newcommand*{\mkboldifhashinlist}[1]{%
  \xifinlist{\thefield{hash}}{\nhblx@boldhashes}
    {\mkbibbold{#1}}
    {#1}}
\makeatother

\DeclareNameWrapperFormat{boldifhashinlist}{%
  \renewcommand*{\mkbibcompletename}{\mkboldifhashinlist}%
  #1}

\DeclareNameWrapperAlias{sortname}{default}
\DeclareNameWrapperAlias{default}{boldifhashinlist}


% only show first and last name
\DeclareNameFormat{FirstLast}{%
  \ifthenelse{\value{listtotal}=1}
    {\namepartgiveni\adddot\addspace\ifblank{\namepartprefix}{}{\namepartprefix\addnbspace}\namepartfamily}
    {\ifthenelse{\value{listtotal}=2}
      {\ifthenelse{\value{listcount}<\value{listtotal}}
        {\namepartgiveni\adddot\addspace\ifblank{\namepartprefix}{}{\namepartprefix\addnbspace}\namepartfamily\addspace}
        {\bibstring{and}\addspace\namepartgiveni\adddot\addspace\ifblank{\namepartprefix}{}{\namepartprefix\addnbspace}\namepartfamily}}
      {\ifthenelse{\value{listcount}=1}
        {\namepartgiveni\adddot\addspace\ifblank{\namepartprefix}{}{\namepartprefix\addnbspace}\namepartfamily\addcomma\addspace\dots\isdot\addcomma}
        {\ifthenelse{\value{listcount}<\value{listtotal}}
          {}
          {\addspace\namepartgiveni\adddot\addspace\ifblank{\namepartprefix}{}{\namepartprefix\addnbspace}\namepartfamily}}%
      }%
    }%
}


% define a prefix for own publications
\DeclareRefcontext{own}{labelprefix=PR}
\DeclareRefcontext{ownpreprint}{labelprefix=PRP}


==> header_tblr.tex <==
\DefTblrTemplate{caption-tag}{nocaption}{}
\SetTblrTemplate{caption-tag}{nocaption}
\DefTblrTemplate{caption-sep}{nocaption}{}
\SetTblrTemplate{caption-sep}{nocaption}
